DEPAC: a Corpus for Depression and Anxiety Detection from Speech

Mental distress like depression and anxiety contribute to the largest proportion of the global burden of diseases. Automated diagnosis systems of such disorders, empowered by recent innovations in Artificial Intelligence, can pave the way to reduce the sufferings of the affected individuals. Development of such systems requires information-rich and balanced corpora. In this work, we introduce a novel mental distress analysis audio dataset DEPAC, labeled based on established thresholds on depression and anxiety standard screening tools. This large dataset comprises multiple speech tasks per individual, as well as relevant demographic information. Alongside, we present a feature set consisting of hand-curated acoustic and linguistic features, which were found effective in identifying signs of mental illnesses in human speech. Finally, we justify the quality and effectiveness of our proposed audio corpus and feature set in predicting depression severity by comparing the performance of baseline machine learning models built on this dataset with baseline models trained on other well-known depression corpora.

==> acl_latex <==
\begin{thebibliography}{66}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[{Akhtar-Danesh and Landeen(2007)}]{akhtar2007relation}
Noori Akhtar-Danesh and Janet Landeen. 2007.
\newblock Relation between depression and sociodemographic factors.
\newblock \emph{International journal of mental health systems}, 1(1):1--9.

\bibitem[{Alpert et~al.(2001)Alpert, Pouget, and Silva}]{alpert2001reflections}
Murray Alpert, Enrique~R Pouget, and Raul~R Silva. 2001.
\newblock Reflections of depression in acoustic measures of the patient’s
  speech.
\newblock \emph{Journal of affective disorders}, 66(1):59--69.

\bibitem[{Bachu et~al.(2008)Bachu, Kopparthi, Adapa, and
  Barkana}]{bachu2008separation}
RG~Bachu, S~Kopparthi, B~Adapa, and BD~Barkana. 2008.
\newblock Separation of voiced and unvoiced using zero crossing rate and energy
  of the speech signal.
\newblock In \emph{American Society for Engineering Education (ASEE) zone
  conference proceedings}, pages 1--7. American Society for Engineering
  Education.

\bibitem[{Barker et~al.(2017)Barker, Young, and Robinson}]{barker2017cohesive}
Megan~S Barker, Breanne Young, and Gail~A Robinson. 2017.
\newblock Cohesive and coherent connected speech deficits in mild stroke.
\newblock \emph{Brain and language}, 168:23--36.

\bibitem[{Beck et~al.(1988)Beck, Steer, and Carbin}]{beck1988psychometric}
Aaron~T Beck, Robert~A Steer, and Margery~G Carbin. 1988.
\newblock Psychometric properties of the beck depression inventory: Twenty-five
  years of evaluation.
\newblock \emph{Clinical psychology review}, 8(1):77--100.

\bibitem[{Berman et~al.(1985)Berman, Miller, and Massman}]{berman1985cognitive}
Jeffrey~S Berman, R~Christopher Miller, and Paul~J Massman. 1985.
\newblock Cognitive therapy versus systematic desensitization: Is one treatment
  superior?
\newblock \emph{Psychological bulletin}, 97(3):451.

\bibitem[{Blanco et~al.(2013)Blanco, Otto, Maddox, Beevers, and
  Love}]{blanco2013influence}
Nathaniel~J Blanco, A~Ross Otto, W~Todd Maddox, Christopher~G Beevers, and
  Bradley~C Love. 2013.
\newblock The influence of depression symptoms on exploratory decision-making.
\newblock \emph{Cognition}, 129(3):563--568.

\bibitem[{Boersma and Van~Heuven(2001)}]{boersma2001speak}
Paul Boersma and Vincent Van~Heuven. 2001.
\newblock Speak and unspeak with praat.
\newblock \emph{Glot International}, 5(9/10):341--347.

\bibitem[{Borkowski et~al.(1967)Borkowski, Benton, and
  Spreen}]{borkowski1967word}
John~G Borkowski, Arthur~L Benton, and Otfried Spreen. 1967.
\newblock Word fluency and brain damage.
\newblock \emph{Neuropsychologia}, 5(2):135--140.

\bibitem[{Brunet et~al.(1978)}]{brunet1978vocabulaire}
{\'E}tienne Brunet et~al. 1978.
\newblock \emph{Le vocabulaire de Jean Giraudoux structure et {\'e}volution}.
\newblock Slatkine.

\bibitem[{Brysbaert and New(2009)}]{brysbaert2009moving}
Marc Brysbaert and Boris New. 2009.
\newblock Moving beyond ku{\v{c}}era and francis: A critical evaluation of
  current word frequency norms and the introduction of a new and improved word
  frequency measure for american english.
\newblock \emph{Behavior research methods}, 41(4):977--990.

\bibitem[{Chae and Nenkova(2009)}]{chae2009predicting}
Jieun Chae and Ani Nenkova. 2009.
\newblock Predicting the fluency of text with shallow structural features: Case
  studies of machine tanslation and human-written text.

\bibitem[{Chandler and Shapiro(2016)}]{chandler2016conducting}
Jesse Chandler and Danielle Shapiro. 2016.
\newblock Conducting clinical research using crowdsourced convenience samples.
\newblock \emph{Annual review of clinical psychology}, 12:53--81.

\bibitem[{Cohen et~al.(1982)Cohen, Weingartner, Smallberg, Pickar, and
  Murphy}]{cohen1982effort}
Robert~M Cohen, Herbert Weingartner, Sheila~A Smallberg, David Pickar, and
  Dennis~L Murphy. 1982.
\newblock Effort and cognition in depression.
\newblock \emph{Archives of general psychiatry}, 39(5):593--597.

\bibitem[{Fineberg et~al.(2016)Fineberg, Leavitt, Deutsch-Link, Dealy, Landry,
  Pirruccio, Shea, Trent, Cecchi, and Corlett}]{fineberg2016self}
Sarah~Kathryn Fineberg, J~Leavitt, Sasha Deutsch-Link, Samson Dealy,
  Christopher~D Landry, Kevin Pirruccio, Samantha Shea, Savannah Trent,
  Guillermo Cecchi, and Philip~R Corlett. 2016.
\newblock Self-reference in psychosis and depression: a language marker of
  illness.
\newblock \emph{Psychological medicine}, 46(12):2605--2615.

\bibitem[{Flint et~al.(1992)Flint, Black, Campbell-Taylor, Gailey, and
  Levinton}]{flint1992acoustic}
Alastair~J Flint, Sandra~E Black, Irene Campbell-Taylor, Gillian~F Gailey, and
  Carey Levinton. 1992.
\newblock Acoustic analysis in the differentiation of parkinson's disease and
  major depression.
\newblock \emph{Journal of Psycholinguistic Research}, 21(5):383--399.

\bibitem[{Forbes-McKay and Venneri(2005)}]{forbes2005detecting}
Katrina~E Forbes-McKay and Annalena Venneri. 2005.
\newblock Detecting subtle spontaneous language decline in early alzheimer’s
  disease with a picture description task.
\newblock \emph{Neurological sciences}, 26(4):243--254.

\bibitem[{Fossati et~al.(2003)Fossati, Ergis, Allilaire
  et~al.}]{fossati2003qualitative}
Philippe Fossati, Anne-Marie Ergis, Jean-Fran{\c{c}}ois Allilaire, et~al. 2003.
\newblock Qualitative analysis of verbal fluency in depression.
\newblock \emph{Psychiatry research}, 117(1):17--24.

\bibitem[{Fraser et~al.(2016)Fraser, Meltzer, and
  Rudzicz}]{fraser2016linguistic}
Kathleen~C Fraser, Jed~A Meltzer, and Frank Rudzicz. 2016.
\newblock Linguistic features identify alzheimer’s disease in narrative
  speech.
\newblock \emph{Journal of Alzheimer's Disease}, 49(2):407--422.

\bibitem[{Galili et~al.(2013)Galili, Amir, and
  Gilboa-Schechtman}]{galili2013acoustic}
Lior Galili, Ofer Amir, and Eva Gilboa-Schechtman. 2013.
\newblock Acoustic properties of dominance and request utterances in social
  anxiety.
\newblock \emph{Journal of social and clinical psychology}, 32(6):651--673.

\bibitem[{Gilboa-Schechtman et~al.(2014)Gilboa-Schechtman, Galili, Sahar, and
  Amir}]{gilboa2014being}
Eva Gilboa-Schechtman, Lior Galili, Yair Sahar, and Ofer Amir. 2014.
\newblock Being “in” or “out” of the game: subjective and acoustic
  reactions to exclusion and popularity in social anxiety.
\newblock \emph{Frontiers in human neuroscience}, 8:147.

\bibitem[{Giles et~al.(1996)Giles, Patterson, and
  Hodges}]{giles1996performance}
Elaine Giles, Karalyn Patterson, and John~R Hodges. 1996.
\newblock Performance on the boston cookie theft picture description task in
  patients with early dementia of the alzheimer's type: missing information.
\newblock \emph{Aphasiology}, 10(4):395--408.

\bibitem[{Goodglass et~al.(2001)Goodglass, Kaplan, and
  Weintraub}]{goodglass2001bdae}
Harold Goodglass, Edith Kaplan, and Sandra Weintraub. 2001.
\newblock \emph{BDAE: The Boston Diagnostic Aphasia Examination}.
\newblock Lippincott Williams \& Wilkins Philadelphia, PA.

\bibitem[{Gratch et~al.(2014)Gratch, Artstein, Lucas, Stratou, Scherer,
  Nazarian, Wood, Boberg, DeVault, Marsella et~al.}]{gratch2014distress}
Jonathan Gratch, Ron Artstein, Gale Lucas, Giota Stratou, Stefan Scherer,
  Angela Nazarian, Rachel Wood, Jill Boberg, David DeVault, Stacy Marsella,
  et~al. 2014.
\newblock The distress analysis interview corpus of human and computer
  interviews.
\newblock In \emph{Proceedings of the Ninth International Conference on
  Language Resources and Evaluation (LREC'14)}, pages 3123--3128.

\bibitem[{Hamilton and Guy(1976)}]{hamilton1976hamilton}
M~Hamilton and W~Guy. 1976.
\newblock Hamilton depression scale.
\newblock \emph{Group}, 1:4.

\bibitem[{Honor{\'e} et~al.(1979)}]{honore1979some}
Antony Honor{\'e} et~al. 1979.
\newblock Some simple measures of richness of vocabulary.
\newblock \emph{Association for literary and linguistic computing bulletin},
  7(2):172--177.

\bibitem[{Howes et~al.(2014)Howes, Purver, and McCabe}]{howes2014linguistic}
Christine Howes, Matthew Purver, and Rose McCabe. 2014.
\newblock Linguistic indicators of severity and progress in online text-based
  therapy for depression.
\newblock In \emph{Proceedings of the workshop on computational linguistics and
  clinical psychology: from linguistic signal to clinical reality}. Association
  for Computational Linguistics.

\bibitem[{Jiang et~al.(2017)Jiang, Hu, Liu, Yan, Wang, Liu, Kang, and
  Li}]{jiang2017investigation}
Haihua Jiang, Bin Hu, Zhenyu Liu, Lihua Yan, Tianyang Wang, Fei Liu, Huanyu
  Kang, and Xiaoyu Li. 2017.
\newblock Investigation of different speech types and emotions for detecting
  depression using different classifiers.
\newblock \emph{Speech Communication}, 90:39--46.

\bibitem[{Kraepelin(1921)}]{kraepelin1921manic}
Emil Kraepelin. 1921.
\newblock Manic depressive insanity and paranoia.
\newblock \emph{The Journal of Nervous and Mental Disease}, 53(4):350.

\bibitem[{Kroenke et~al.(2001)Kroenke, Spitzer, and Williams}]{kroenke2001phq}
Kurt Kroenke, Robert~L Spitzer, and Janet~BW Williams. 2001.
\newblock The phq-9: validity of a brief depression severity measure.
\newblock \emph{Journal of general internal medicine}, 16(9):606--613.

\bibitem[{Leung et~al.(2009)Leung, Lee, Yip, Li, and Wong}]{leung2009selective}
Kwok-Keung Leung, Tatia~MC Lee, Paul Yip, Leonard~SW Li, and Michael~MC Wong.
  2009.
\newblock Selective attention biases of people with depression: Positive and
  negative priming of depression-related information.
\newblock \emph{Psychiatry research}, 165(3):241--251.

\bibitem[{Low et~al.(2020)Low, Bentley, and Ghosh}]{low2020automated}
Daniel~M Low, Kate~H Bentley, and Satrajit~S Ghosh. 2020.
\newblock Automated assessment of psychiatric disorders using speech: A
  systematic review.
\newblock \emph{Laryngoscope Investigative Otolaryngology}, 5(1):96--116.

\bibitem[{L{\"o}we et~al.(2004)L{\"o}we, Un{\"u}tzer, Callahan, Perkins, and
  Kroenke}]{lowe2004monitoring}
Bernd L{\"o}we, J{\"u}rgen Un{\"u}tzer, Christopher~M Callahan, Anthony~J
  Perkins, and Kurt Kroenke. 2004.
\newblock Monitoring depression treatment outcomes with the patient health
  questionnaire-9.
\newblock \emph{Medical care}, pages 1194--1201.

\bibitem[{Lu(2010)}]{lu2010automatic}
Xiaofei Lu. 2010.
\newblock Automatic analysis of syntactic complexity in second language
  writing.
\newblock \emph{International journal of corpus linguistics}, 15(4):474--496.

\bibitem[{MacWhinney(2000)}]{macwhinney2000childes}
Brian MacWhinney. 2000.
\newblock The childes project: Tools for analyzing talk: Volume i:
  Transcription format and programs, volume ii: The database.

\bibitem[{MacWhinney(2007)}]{macwhinney2007talkbank}
Brian MacWhinney. 2007.
\newblock The talkbank project.
\newblock In \emph{Creating and digitizing language corpora}, pages 163--180.
  Springer.

\bibitem[{Mathews and MacLeod(2005)}]{mathews2005cognitive}
Andrew Mathews and Colin MacLeod. 2005.
\newblock Cognitive vulnerability to emotional disorders.
\newblock \emph{Annu. Rev. Clin. Psychol.}, 1:167--195.

\bibitem[{Mikolov et~al.(2013)Mikolov, Sutskever, Chen, Corrado, and
  Dean}]{mikolov2013distributed}
Tomas Mikolov, Ilya Sutskever, Kai Chen, Greg~S Corrado, and Jeff Dean. 2013.
\newblock Distributed representations of words and phrases and their
  compositionality.
\newblock In \emph{Advances in neural information processing systems}, pages
  3111--3119.

\bibitem[{Montgomery and {\AA}sberg(1979)}]{montgomery1979new}
Stuart~A Montgomery and MARIE {\AA}sberg. 1979.
\newblock A new depression scale designed to be sensitive to change.
\newblock \emph{The British journal of psychiatry}, 134(4):382--389.

\bibitem[{Mota et~al.(2012)Mota, Vasconcelos, Lemos, Pieretti, Kinouchi,
  Cecchi, Copelli, and Ribeiro}]{mota2012speech}
Natalia~B Mota, Nivaldo~AP Vasconcelos, Nathalia Lemos, Ana~C Pieretti, Osame
  Kinouchi, Guillermo~A Cecchi, Mauro Copelli, and Sidarta Ribeiro. 2012.
\newblock Speech graphs provide a quantitative measure of thought disorder in
  psychosis.
\newblock \emph{PloS one}, 7(4):e34928.

\bibitem[{Mundt et~al.(2007)Mundt, Snyder, Cannizzaro, Chappie, and
  Geralts}]{mundt2007voice}
James~C Mundt, Peter~J Snyder, Michael~S Cannizzaro, Kara Chappie, and Dayna~S
  Geralts. 2007.
\newblock Voice acoustic measures of depression severity and treatment response
  collected via interactive voice response (ivr) technology.
\newblock \emph{Journal of neurolinguistics}, 20(1):50--64.

\bibitem[{Nemeroff(2007)}]{nemeroff2007prevalence}
Charles~B Nemeroff. 2007.
\newblock Prevalence and management of treatment-resistant depression.
\newblock \emph{Journal of Clinical Psychiatry}, 68(8):17.

\bibitem[{Paolacci et~al.(2010)Paolacci, Chandler, and
  Ipeirotis}]{paolacci2010running}
Gabriele Paolacci, Jesse Chandler, and Panagiotis~G Ipeirotis. 2010.
\newblock Running experiments on amazon mechanical turk.
\newblock \emph{Judgment and Decision making}, 5(5):411--419.

\bibitem[{Patel and Connaghan(2014)}]{patel2014park}
Rupal Patel and Kathryn Connaghan. 2014.
\newblock Park play: A picture description task for assessing childhood motor
  speech disorders.
\newblock \emph{International Journal of Speech-Language Pathology},
  16(4):337--343.

\bibitem[{Pedregosa et~al.(2011)Pedregosa, Varoquaux, Gramfort, Michel,
  Thirion, Grisel, Blondel, Prettenhofer, Weiss, Dubourg, Vanderplas, Passos,
  Cournapeau, Brucher, Perrot, and Duchesnay}]{scikit-learn}
F.~Pedregosa, G.~Varoquaux, A.~Gramfort, V.~Michel, B.~Thirion, O.~Grisel,
  M.~Blondel, P.~Prettenhofer, R.~Weiss, V.~Dubourg, J.~Vanderplas, A.~Passos,
  D.~Cournapeau, M.~Brucher, M.~Perrot, and E.~Duchesnay. 2011.
\newblock Scikit-learn: Machine learning in {P}ython.
\newblock \emph{Journal of Machine Learning Research}, 12:2825--2830.

\bibitem[{Pennington et~al.(2014)Pennington, Socher, and
  Manning}]{pennington2014glove}
Jeffrey Pennington, Richard Socher, and Christopher~D Manning. 2014.
\newblock Glove: Global vectors for word representation.
\newblock In \emph{Proceedings of the 2014 conference on empirical methods in
  natural language processing (EMNLP)}, pages 1532--1543.

\bibitem[{Pope et~al.(1970)Pope, Blass, Siegman, and Raher}]{pope1970anxiety}
Benjamin Pope, Thomas Blass, Aron~W Siegman, and Jack Raher. 1970.
\newblock Anxiety and depression in speech.
\newblock \emph{Journal of Consulting and Clinical Psychology}, 35(1p1):128.

\bibitem[{Quatieri and Malyska(2012)}]{quatieri2012vocal}
Thomas~F Quatieri and Nicolas Malyska. 2012.
\newblock Vocal-source biomarkers for depression: A link to psychomotor
  activity.
\newblock In \emph{Thirteenth annual conference of the international speech
  communication association}.

\bibitem[{Ray et~al.(2019)Ray, Kumar, Reddy, Mukherjee, and
  Garg}]{ray2019multi}
Anupama Ray, Siddharth Kumar, Rutvik Reddy, Prerana Mukherjee, and Ritu Garg.
  2019.
\newblock Multi-level attention network using text, audio and video for
  depression prediction.
\newblock In \emph{Proceedings of the 9th international on audio/visual emotion
  challenge and workshop}, pages 81--88.

\bibitem[{Rejaibi et~al.(2022)Rejaibi, Komaty, Meriaudeau, Agrebi, and
  Othmani}]{rejaibi2022mfcc}
Emna Rejaibi, Ali Komaty, Fabrice Meriaudeau, Said Agrebi, and Alice Othmani.
  2022.
\newblock Mfcc-based recurrent neural network for automatic clinical depression
  recognition and assessment from speech.
\newblock \emph{Biomedical Signal Processing and Control}, 71:103107.

\bibitem[{Ringeval et~al.(2019)Ringeval, Schuller, Valstar, Cummins, Cowie,
  Tavabi, Schmitt, Alisamir, Amiriparian, Messner et~al.}]{ringeval2019avec}
Fabien Ringeval, Bj{\"o}rn Schuller, Michel Valstar, Nicholas Cummins, Roddy
  Cowie, Leili Tavabi, Maximilian Schmitt, Sina Alisamir, Shahin Amiriparian,
  Eva-Maria Messner, et~al. 2019.
\newblock Avec 2019 workshop and challenge: state-of-mind, detecting depression
  with ai, and cross-cultural affect recognition.
\newblock In \emph{Proceedings of the 9th International on Audio/Visual Emotion
  Challenge and Workshop}, pages 3--12.

\bibitem[{Ringeval et~al.(2017)Ringeval, Schuller, Valstar, Gratch, Cowie,
  Scherer, Mozgai, Cummins, Schmitt, and Pantic}]{ringeval2017avec}
Fabien Ringeval, Bj{\"o}rn Schuller, Michel Valstar, Jonathan Gratch, Roddy
  Cowie, Stefan Scherer, Sharon Mozgai, Nicholas Cummins, Maximilian Schmitt,
  and Maja Pantic. 2017.
\newblock Avec 2017: Real-life depression, and affect recognition workshop and
  challenge.
\newblock In \emph{Proceedings of the 7th Annual Workshop on Audio/Visual
  Emotion Challenge}, pages 3--9.

\bibitem[{Shin et~al.(2021)Shin, Cho, Park, Rhee, Kim, Lee, Kim, and
  Ahn}]{shin2021detection}
Daun Shin, Won~Ik Cho, C~Hyung~Keun Park, Sang~Jin Rhee, Min~Ji Kim, Hyunju
  Lee, Nam~Soo Kim, and Yong~Min Ahn. 2021.
\newblock Detection of minor and major depression through voice as a biomarker
  using machine learning.
\newblock \emph{Journal of clinical medicine}, 10(14):3046.

\bibitem[{Smirnova et~al.(2018)Smirnova, Cumming, Sloeva, Kuvshinova, Romanov,
  and Nosachev}]{smirnova2018language}
Daria Smirnova, Paul Cumming, Elena Sloeva, Natalia Kuvshinova, Dmitry Romanov,
  and Gennadii Nosachev. 2018.
\newblock Language patterns discriminate mild depression from normal sadness
  and euthymic state.
\newblock \emph{Frontiers in psychiatry}, 9:105.

\bibitem[{Snyder et~al.(2014)Snyder, Kaiser, Whisman, Turner, Guild, and
  Munakata}]{snyder2014opposite}
Hannah~R Snyder, Roselinde~H Kaiser, Mark~A Whisman, Amy~EJ Turner, Ryan~M
  Guild, and Yuko Munakata. 2014.
\newblock Opposite effects of anxiety and depressive symptoms on executive
  function: The case of selecting among competing options.
\newblock \emph{Cognition \& emotion}, 28(5):893--902.

\bibitem[{Spitzer et~al.(2006)Spitzer, Kroenke, Williams, and
  L{\"o}we}]{spitzer2006brief}
Robert~L Spitzer, Kurt Kroenke, Janet~BW Williams, and Bernd L{\"o}we. 2006.
\newblock A brief measure for assessing generalized anxiety disorder: the
  gad-7.
\newblock \emph{Archives of internal medicine}, 166(10):1092--1097.

\bibitem[{Stadthagen-Gonzalez and Davis(2006)}]{stadthagen2006bristol}
Hans Stadthagen-Gonzalez and Colin~J Davis. 2006.
\newblock The bristol norms for age of acquisition, imageability, and
  familiarity.
\newblock \emph{Behavior research methods}, 38(4):598--605.

\bibitem[{Trifu et~al.(2017)Trifu, NEME{\c{S}}, Bodea-Hațegan, and
  Cozman}]{trifu2017linguistic}
Raluca~Nicoleta Trifu, Bogdan NEME{\c{S}}, Carolina Bodea-Hațegan, and Doina
  Cozman. 2017.
\newblock Linguistic indicators of language in major depressive disorder (mdd).
  an evidence based research.
\newblock \emph{Journal of Evidence-Based Psychotherapies}, 17(1).

\bibitem[{Valstar et~al.(2016)Valstar, Gratch, Schuller, Ringeval, Lalanne,
  Torres~Torres, Scherer, Stratou, Cowie, and Pantic}]{valstar2016avec}
Michel Valstar, Jonathan Gratch, Bj{\"o}rn Schuller, Fabien Ringeval, Denis
  Lalanne, Mercedes Torres~Torres, Stefan Scherer, Giota Stratou, Roddy Cowie,
  and Maja Pantic. 2016.
\newblock Avec 2016: Depression, mood, and emotion recognition workshop and
  challenge.
\newblock In \emph{Proceedings of the 6th international workshop on
  audio/visual emotion challenge}, pages 3--10.

\bibitem[{Valstar et~al.(2014)Valstar, Schuller, Smith, Almaev, Eyben,
  Krajewski, Cowie, and Pantic}]{valstar2014avec}
Michel Valstar, Bj{\"o}rn Schuller, Kirsty Smith, Timur Almaev, Florian Eyben,
  Jarek Krajewski, Roddy Cowie, and Maja Pantic. 2014.
\newblock Avec 2014: 3d dimensional affect and depression recognition
  challenge.
\newblock In \emph{Proceedings of the 4th international workshop on
  audio/visual emotion challenge}, pages 3--10.

\bibitem[{Valstar et~al.(2013)Valstar, Schuller, Smith, Eyben, Jiang, Bilakhia,
  Schnieder, Cowie, and Pantic}]{valstar2013avec}
Michel Valstar, Bj{\"o}rn Schuller, Kirsty Smith, Florian Eyben, Bihan Jiang,
  Sanjay Bilakhia, Sebastian Schnieder, Roddy Cowie, and Maja Pantic. 2013.
\newblock Avec 2013: the continuous audio/visual emotion and depression
  recognition challenge.
\newblock In \emph{Proceedings of the 3rd ACM international workshop on
  Audio/visual emotion challenge}, pages 3--10.

\bibitem[{Wakefield(2013)}]{wakefield2013dsm}
Jerome~C Wakefield. 2013.
\newblock The dsm-5 debate over the bereavement exclusion: Psychiatric
  diagnosis and the future of empirically supported treatment.
\newblock \emph{Clinical psychology review}, 33(7):825--845.

\bibitem[{Warriner et~al.(2013)Warriner, Kuperman, and
  Brysbaert}]{warriner2013norms}
Amy~Beth Warriner, Victor Kuperman, and Marc Brysbaert. 2013.
\newblock Norms of valence, arousal, and dominance for 13,915 english lemmas.
\newblock \emph{Behavior research methods}, 45(4):1191--1207.

\bibitem[{Yngve(1960)}]{yngve1960model}
Victor~H Yngve. 1960.
\newblock A model and an hypothesis for language structure.
\newblock \emph{Proceedings of the American philosophical society},
  104(5):444--466.

\bibitem[{Zinken et~al.(2010)Zinken, Zinken, Wilson, Butler, and
  Skinner}]{zinken2010analysis}
J{\"o}rg Zinken, Katarzyna Zinken, J~Clare Wilson, Lisa Butler, and Timothy
  Skinner. 2010.
\newblock Analysis of syntax and word use to predict successful participation
  in guided self-help for anxiety and depression.
\newblock \emph{Psychiatry research}, 179(2):181--186.

\bibitem[{Zucco et~al.(2017)Zucco, Calabrese, and
  Cannataro}]{zucco2017sentiment}
Chiara Zucco, Barbara Calabrese, and Mario Cannataro. 2017.
\newblock Sentiment analysis and affective computing for depression monitoring.
\newblock In \emph{2017 IEEE international conference on bioinformatics and
  biomedicine (BIBM)}, pages 1988--1995. IEEE.

\end{thebibliography}

